Improving Medical Visual Representations via Radiology Report Generation

Vision-language pretraining has been shown to produce high-quality visual encoders which transfer efficiently to downstream computer vision tasks. Contrastive learning approaches have increasingly been adopted for medical vision language pretraining (MVLP), yet recent developments in generative AI offer new modeling alternatives. This paper introduces RadTex, a CNN-encoder transformer-decoder architecture optimized for radiology. We explore bidirectional captioning as an alternative MVLP strategy and demonstrate that RadTex's captioning pretraining is competitive with established contrastive methods, achieving a CheXpert macro-AUC of 89.4%. Additionally, RadTex's lightweight text decoder not only generates clinically relevant radiology reports (macro-F1 score of 0.349), but also provides targeted, interactive responses, highlighting the utility of bidirectional captioning in advancing medical image analysis.

==> sections/disc.tex <==
% We find bidirectional captioning pretraining to be an effective alternative to contrastive pretraining for learning transferable visual representations in radiology. Comparing to contrastive baselines with similar model sizes and pretraining datasets, RadTex exhibits superior performance on three of four major downstream visual tasks. RadTex also shows improved data efficiency and fine-grained image classification abilities, aligning with the growing needs of radiologists.

% We freeze the visual encoder in transferred tasks in an effort to isolate the benefits of self-supervised pretraining.

% We propose two hypotheses for the success of RadTex pretraining. First, contrastive learning may inadvertently classify similar examples as dissimilar, potentially leading to false negatives \cite{huynh2022boosting}, a critical issue given the semantic similarity often displayed in radiographic images. Captioning models, in contrast, can encode these hard negatives without artificially enforcing dissimilarity. Second, while traditional contrastive learning primarily captures high-level global semantics of images and text, diagnostic tasks often require finer-grained understanding of images \cite{wang2022multi}. RadTex, using a token-level loss function and bidirectional causal masking, effectively utilizes the dense semantics of text to capture fine-grained image features important for effective diagnostics. 


% RadTex's superior performance on COVIDx and EdemaSeverity tasks further supports these hypotheses. The classification of COVID-19, identified three years after the latest examples in MIMIC-CXR \cite{johnson_mimic-cxr_2019}, requires the encoding of fine-grained symptoms which may be out-of-distribution from the pretraining dataset. On the EdemaSeverity task, radiologists find differentiating between vascular congestion and interstitial edema (1 vs 2) more challenging than distinguishing  interstitial from alveolar edema (2 vs 3). RadTex's superior differentiation of the former reflects the fine-grained representations learned during pretraining.




% While contrastive methods have shown remarkable success in X-ray image analysis, they often lack interpretability, a critical aspect for fostering transparency, clinical workflow integration, and finally clinician acceptance. A system capable of generating radiology reports with detailed pathological findings alongside classifications would align well with physicians' workflows, streamlining the reporting process and improving healthcare outcomes. 
% The COVID-19 virus and its symptoms were identified three years after the latest examples in MIMIC-CXR \cite{johnson_mimic-cxr_2019}, meaning that its classification requires the encoding of fine-grained symptoms which may be out-of-distribution from the pretraining dataset. On the EdemaSeverity task (gradings of 0-3), radiologists assess the differentiation between vascular congestion and interstitial edema as more difficult than the differentiation between interstial and alveolar edema. We believe RadTex's superior differentiation of the former reflects the fine-grained representations learned during pretraining.

% Given the substantial variability in pathology appearance and overlap between normal and pathological findings, diagnosis based on imaging alone can sometimes be impossible. This challenge can be addressed by a system capable of generating radiology reports with detailed
% pathological findings alongside classifications. Such a system would align well with physicians’ workflows, streamlining
% the reporting process, leading to greater efficiency, consistency, and improving healthcare outcomes.

% \subsection{Limitations}
% CheXzero was motivated by a need for zero-shot classification of CXR, and they reported impressive zero-shot performance on CheXpert Competition (macro-AUC of 88.9\%). We found no significant performance change with linear finetuning (macro-AUC of 88.9\% @ 1\%, 89.0\% @ 100\%), a testament to the strengths of contrastive pretraining for zero-shot pathology classification, which has no direct analogue with captioning pretraining. However, given the bicaptioning pretraining performance improvements, future work should look at the fusion of contrastive and captioning objectives for radiology, where training objectives may be complementary.

% We studied downstream performance on mainly classification tasks. While these tasks were diverse, further research is needed to demonstrate transferability of pretrained visual models to additional tasks (e.g. object detection).

% In Sec~\ref{sec:hallucinations}, we describe the challenges of hallucination when prompting. The inability to negate pathologies mentioned in a prompt (e.g. ``Atelectasis...is not present.") may be a symptom of larger challenges with captioning systems, which must consider both image and text priors when generating tokens. Yang \etal \cite{yang2023ig} observed that such systems can ignore image features and generate solely based on text priors in the natural domain, proposing an information gain solution to improve zero-shot classification of captioning models. We leave exploration of this pretraining modification in radiology to future work.


% Points of discussion:
% \begin{itemize}
%     \item Superior performance to CheXzero--reasons for why...(findings similar to those of MedPaLM M)
%     \item Fine-grained medical semantics encoded--discuss shuffling experiment and rehash differences between natural domain and medical domain. Mention IG Captioner and the potential for future research
%     \item Other works cite a CNN-transformer architecture--what makes ours different?
%     \item Fine-grained medical semantics: EdemaSeverity as a proxy. 
%     To test our hypothesis that 
%     \item discussion of chexzero zero shot vs linear performance vs RRG (interesting observation...when might zero-shot be preferable?)
%     \item Why does Supervised do better on COVIDx?
%     \item "In clinical practice, the chest radiograph is just one [tool] used in developing a diagnosis."
%     \item Doing better than MedPaLM M on our one overlapping task--still a need for domain-specific models
%     \item: future work: scaling our approach (expect improvement in captioning given MedPaLM M, should we expect similar for classification?), adding additional losses like IG Captioner to improve RRG specificity?
% \end{itemize}

% \subsection{Limitations}
% \begin{itemize}
%     \item Ability to do zero-shot classification
%     \item Hallucinations when prompted naively (adding names of all pathologies). The RRG module has a difficult time with negation
%     \item Evaluation on localized data 
%     \item Not ready for prime-time
% \end{itemize}
% Vitae: Vision transformer advanced by exploring intrinsic inductive bias.  Vision transfomers lack the inductive biases necessary for accurate modeling
